The End of Trust: How Agentic AI Breaks Security Assumptions

For decades, the security of digital interaction has rested on an unacknowledged economic constraint. Attackers faced a tradeoff between the fidelity of a deception and the scale at which it could be deployed. Convincing impersonation required sustained human effort and was confined to a narrow set of high-value targets, while mass-market attacks sacrificed plausibility for reach. Detection systems, verification mechanisms, and user awareness training have all been implicitly calibrated to the artifacts of cheap deception that this tradeoff produced. Agentic AI collapses the tradeoff, allowing high-fidelity, individually tailored deception to be produced at mass-market scale. We argue that this shift exhausts a security paradigm rather than merely intensifying the threat landscape. We introduce the Infinite Impostor, an attack model in which an autonomous agent interposes itself between two parties who already trust each other, hijacking an existing relationship rather than building a new one from scratch. Detection-oriented defenses share an assumption that generative progress is eliminating, that synthetic outputs are distinguishable from authentic ones. We propose a suspect-by-default paradigm that shifts security from authenticating actors to evaluating actions, and examine the governance tensions that arise when platforms become the regulatory substrate of digital interaction.

==> FigTex/FigInfiniteImposters.tex <==

% =====================================================================
%  FIGURE --- SINGLE COLUMN (compact)
%  The Infinite Impostor
% =====================================================================

\begin{tikzpicture}
    \useasboundingbox (0.3,1.4) rectangle (8.2,8.25);
    % \fill[paperBG,rounded corners=3pt] (0,0) rectangle (8.6,9.6);

    % ---------- Title ----------
    % \node[font=\sffamily\bfseries\small,text=darkGray,align=center,text width=8.2cm]
    %     at (4.3,9.05)
    %     {The Infinite Impostor: \\ Hijacking an Existing Trust Relationship};

    % ---------- Pre-existing trust: green ribbon between Alice and Bob (background layer) ----------
    \begin{scope}[on background layer]
        \draw[safeGreen!55,line width=3mm,line cap=round,opacity=0.5]
            (2.10,5.80) -- (6.50,5.80);
    \end{scope}
    % Small inline annotation (placed on a clear left segment of the ribbon)
    \node[font=\sffamily\scriptsize\itshape,text=safeGreenDark,
          fill=paperBG,inner sep=1.5pt,rounded corners=2pt,anchor=center]
        at (2.75,5.80) {trust};
    \node[font=\sffamily\scriptsize\itshape,text=safeGreenDark,
          fill=paperBG,inner sep=1.5pt,rounded corners=2pt,anchor=center]
        at (5.85,5.80) {trust};

    % ---------- Alice (left) ----------
    \node[circle,fill=trustBlueLight,draw=trustBlue,line width=0.5mm,
          minimum size=1.45cm,inner sep=0pt] (alice) at (1.40,5.80) {};
    \node[text=trustBlue] at (alice) {\LARGE\faUserCircle};
    \node[font=\sffamily\bfseries\small,text=trustBlue] at (1.40,4.85) {Alice};
    \node[font=\sffamily\scriptsize\itshape,text=darkGray!85,align=center,
          text width=2.6cm] at (1.40,4.30) {believes she is \\ talking to Bob};

    % ---------- Bob (right) ----------
    \node[circle,fill=trustBlueLight,draw=trustBlue,line width=0.5mm,
          minimum size=1.45cm,inner sep=0pt] (bob) at (7.20,5.80) {};
    \node[text=trustBlue] at (bob) {\LARGE\faUserCircle};
    \node[font=\sffamily\bfseries\small,text=trustBlue] at (7.20,4.85) {Bob};
    \node[font=\sffamily\scriptsize\itshape,text=darkGray!85,align=center,
          text width=2.6cm] at (7.20,4.30) {believes he is \\ talking to Alice};

    % ---------- Central agent (hexagon + glow) ----------
    \begin{scope}[on background layer]
        \foreach \r/\op in {1.20/0.05, 1.00/0.10, 0.85/0.18, 0.72/0.26}
            \fill[dangerRed,opacity=\op] (4.30,5.80) circle (\r);
    \end{scope}
    \node[regular polygon,regular polygon sides=6,
          fill=dangerRedDark,draw=dangerRed,line width=0.55mm,
          minimum size=1.6cm,inner sep=0pt] (agent) at (4.30,5.80) {};
    \node[text=sunYellow] at (4.30,5.92) {\Large\faRobot};
    \node[font=\sffamily\bfseries\scriptsize,text=white] at (4.30,5.38) {Agent};

    % ---------- Ghost persona "Bob" that Alice sees (above) ----------
    \node[rounded corners=4pt,draw=aiPurple,fill=aiPurple!12,
          line width=0.4mm,dashed,dash pattern=on 2.5pt off 1.5pt,
          minimum width=1.9cm,minimum height=0.85cm,inner sep=0pt]
        (fakebob) at (2.70,7.55) {};
    \node[text=aiPurple,anchor=west] at (1.85,7.55) {\small\faUserSecret};
    \node[font=\sffamily\bfseries\footnotesize,text=aiPurple,anchor=west]
        at (2.40,7.55) {``Bob''};

    % ---------- Ghost persona "Alice" that Bob sees (above) ----------
    \node[rounded corners=4pt,draw=aiPurple,fill=aiPurple!12,
          line width=0.4mm,dashed,dash pattern=on 2.5pt off 1.5pt,
          minimum width=1.9cm,minimum height=0.85cm,inner sep=0pt]
        (fakealice) at (5.90,7.55) {};
    \node[text=aiPurple,anchor=west] at (5.05,7.55) {\small\faUserSecret};
    \node[font=\sffamily\bfseries\footnotesize,text=aiPurple,anchor=west]
        at (5.60,7.55) {``Alice''};

    % Small descriptive tags for the ghosts (kept short, placed above the boxes)
    \node[font=\sffamily\scriptsize\itshape,text=aiPurple!85!black,anchor=south]
        at (2.70,8.05) {persona shown to Alice};
    \node[font=\sffamily\scriptsize\itshape,text=aiPurple!85!black,anchor=south]
        at (5.90,8.05) {persona shown to Bob};

    % ---------- Visible conversation arrows (solid blue, bidirectional) ----------
    \draw[{Stealth[length=2.3mm]}-{Stealth[length=2.3mm]},
          trustBlue,line width=0.55mm] (alice) -- (fakebob);
    \draw[{Stealth[length=2.3mm]}-{Stealth[length=2.3mm]},
          trustBlue,line width=0.55mm] (bob) -- (fakealice);

    % ---------- Hidden relay arrows (dashed red) ----------
    \draw[{Stealth[length=2mm]}-{Stealth[length=2mm]},
          dangerRed,line width=0.45mm,dashed,dash pattern=on 2.5pt off 1.5pt]
        (fakebob) -- (agent);
    \draw[{Stealth[length=2mm]}-{Stealth[length=2mm]},
          dangerRed,line width=0.45mm,dashed,dash pattern=on 2.5pt off 1.5pt]
        (fakealice) -- (agent);

    % ---------- Sparkles around the agent (alive feel) ----------
    \node[text=sunYellow,font=\tiny] at (3.50,6.55) {\faStarOfLife};
    \node[text=sunYellow,font=\tiny] at (5.10,6.55) {\faStarOfLife};

    % ---------- Harvesting channel (agent south -> downward) ----------
    \draw[-{Stealth[length=3.5mm,width=3mm]},dangerRed,line width=0.9mm]
        (agent.south) -- (4.30,3.55);
    \node[font=\sffamily\bfseries\footnotesize,text=dangerRed,
          fill=paperBG,inner sep=2pt] at (4.30,3.85) {silently harvested};

    % ---------- Data chips ----------
    \foreach \x/\ic/\lab in {
        1.40/faKey/credentials,
        3.40/faEnvelopeOpen/messages,
        5.30/faDollarSign/payments,
        7.10/faIdCard/{PII / KYC}%
    }{
        \node[rounded corners=4pt,fill=dangerRed!12,draw=dangerRed,line width=0.35mm,
              minimum width=1.6cm,minimum height=0.85cm,inner sep=0pt]
            at (\x,2.20) {};
        \node[text=dangerRed] at (\x,2.35) {\small\csname\ic\endcsname};
        \node[font=\sffamily\scriptsize\bfseries,text=dangerRed!70!black]
            at (\x,1.99) {\lab};
    }

    % Fan-in connecting the harvest channel to each chip
    \foreach \x in {1.40, 3.40, 5.30, 7.10}{
        \draw[dangerRed!50,line width=0.3mm,dashed,dash pattern=on 1.5pt off 1.5pt]
            (4.30,3.45) -- (\x,2.65);
    }
\end{tikzpicture}


